JiuZhang3.0: Efficiently Improving Mathematical Reasoning by Training Small Data Synthesis Models

Mathematical reasoning is an important capability of large language models~(LLMs) for real-world applications. To enhance this capability, existing work either collects large-scale math-related texts for pre-training, or relies on stronger LLMs (\eg GPT-4) to synthesize massive math problems. Both types of work generally lead to large costs in training or synthesis. To reduce the cost, based on open-source available texts, we propose an efficient way that trains a small LLM for math problem synthesis, to efficiently generate sufficient high-quality pre-training data. To achieve it, we create a dataset using GPT-4 to distill its data synthesis capability into the small LLM. Concretely, we craft a set of prompts based on human education stages to guide GPT-4, to synthesize problems covering diverse math knowledge and difficulty levels. Besides, we adopt the gradient-based influence estimation method to select the most valuable math-related texts. The both are fed into GPT-4 for creating the knowledge distillation dataset to train the small LLM. We leverage it to synthesize 6 million math problems for pre-training our JiuZhang3.0 model, which only needs to invoke GPT-4 API 9.3k times and pre-train on 4.6B data. Experimental results have shown that JiuZhang3.0 achieves state-of-the-art performance on several mathematical reasoning datasets, under both natural language reasoning and tool manipulation settings. Our code and data will be publicly released in \url{https://github.com/RUCAIBox/JiuZhang3.0}.

==> prompts/cot/amc10.tex <==
\textbf{Instruction}

Inspired by the math content, craft a math problem suitable for the AMC 10 competition, challenging students with interests in areas such as arithmetic, algebra, geometry, counting, probability, and number theory. The problem should be challenging but not as difficult as the hardest problems in the competition. It should foster advanced problem-solving skills and mathematical reasoning, without crossing into advanced math (such as calculus) or physics.
\\

\textbf{Math Content}

[Math Text Placeholder]
\\

\textbf{Guidelines}

[Problem]: Create an intriguing and challenging math problem for AMC 10 contestants inspired by the math content, integrating aspects of intermediate math disciplines. The problem should prompt students to apply higher-level logical reasoning and problem-solving strategies. The problem must be text-based and solvable without the need for diagrams. Aim for a problem statement of approximately 50-100 words.

[Solution]: Offer a detailed, step-by-step solution that educates and is tailored to the AMC 10 level, around 250-350 words long. Clearly explain the thought process and methodologies behind each step, using language that is understandable yet challenges students to think deeply. The solution should be concise, with a target length of 150-300 words.
Ensure that the problem statement is unambiguous and provides sufficient information for a unique solution. Include a mix of problem types, such as proof-based problems, computation-based problems, or problems that require creative insights.

